Is Vanilla Policy Gradient Overlooked? Analyzing Deep Reinforcement Learning for Hanabi

In pursuit of enhanced multi-agent collaboration, we analyze several on-policy deep reinforcement learning algorithms in the recently published Hanabi benchmark. Our research suggests a perhaps counter-intuitive finding, where Proximal Policy Optimization (PPO) is outperformed by Vanilla Policy Gradient over multiple random seeds in a simplified environment of the multi-agent cooperative card game. In our analysis of this behavior we look into Hanabi-specific metrics and hypothesize a reason for PPO's plateau. In addition, we provide proofs for the maximum length of a perfect game (71 turns) and any game (89 turns). Our code can be found at: https://github.com/bramgrooten/DeepRL-for-Hanabi

==> sections/a-proof89.tex <==

\section{Part 2 of the proof of Proposition~\ref{89}}
\label{sec:proof89}

Let us repeat the proposition:
\begin{proposition*}
The maximum length of a Hanabi game is 89 turns.
\end{proposition*}


\begin{proof}
\textit{Part 1.} See Section \ref{sec:game-length} for the first part of this proof.

\textit{Part 2.} 
In this part we define a value $\Sigma_t$ for a Hanabi game. We will show that it is impossible for this value to increase during the game ($\Sigma_{t+1} \leq \Sigma_{t} \ \forall t$) from which the maximum number of turns follows. 
% The value $\Sigma_t$ can be interpreted as the maximum possible number of total turns that is still reachable, after time step $t$.
We first define a few values: % in Table \ref{tab:hanabi-values}.

% \begin{table}[H]
%     \centering
%     \caption{Defined values of a Hanabi game.}
%     \label{tab:hanabi-values}
\begin{center}
    \begin{tabular}{cl}%\toprule
        % Value & Definition \\ \midrule
        $t$ & total number of turns taken  \\
        $d_t$ & deck size after turn $t$ \\
        $m_t$ & hint tokens left over after turn $t$ \\ %\bottomrule
    \end{tabular}
\end{center}
% \end{table}
% We denote the current total number of turns taken by $t$, and the current deck size after turn $t$ by $d_t$. 
We further define $c_t$, which stands for the number of hint tokens left over after turn $t$, but with the restriction that these tokens can still be used before the deck is empty:
\begin{equation}\label{ctdef}
    c_t = \begin{cases}
    m_t & \text{ if } d_t > 0,\\
    0 & \text{ if } d_t = 0.
    \end{cases}
\end{equation}
% Recall from Section \ref{sec:math-han} that $m_t$ is the number of hint tokens available, without any restrictions.
We add the restriction to $c_t$ here to distinguish between the situations before and after the deck has been emptied. Once the deck is empty, hint actions cannot be used to stall the game anymore. When $d_t = 0$, there is a fixed maximum number of turns left, which we denote by $p_t$ (initially equal to the number of players $p$). 

We define one more value: $u_t$, which we call the \textit{undisclosed hints}. This value counts the number of cards that can still retrieve a hint token which can be used before the deck is empty. We have:
\begin{equation}\label{utdef}
    u_t = \begin{cases}
    d_t - 1 & \text{ if } d_t > 0,\\
    0 & \text{ if } d_t = 0.
    \end{cases}
\end{equation}
Every card that is played or discarded can retrieve a hint token. This can be done $d_0$ times in total and then the deck is empty. However, if the last card that empties the deck retrieves a hint token, this token is only usable after the deck is empty. Thus, the value of $u_t$ is always one less than the current deck size $d_t$ (except when the deck is already empty).

Our $\Sigma_t$ is now defined as the sum over these previous values:
\begin{equation}\label{eq:sigmat}
    \Sigma_t = t + c_t + d_t + u_t + p_t
\end{equation}
and can be interpreted as the maximum possible number of total turns that is still reachable, after time step $t$.

%%% The following command should be issued somewhere in the first column 
%%% of the final page of your paper.
\balance

We will now look into the effect of different actions on the values of $t$, $c_t$, $d_t$, $u_t$, $p_t$, and thus $\Sigma_t$.
A player can choose three actions in each turn: play, discard, or hint. The effect of each action on the different values is summarized in Table \ref{tab:action-effects}.
% Notice that with every \textit{play} or \textit{discard} action the number of undisclosed hints decreases by one: $u_t = u_{t-1} - 1$, as there is one less card available to retrieve a hint token from. We denote this change as $\Delta u_t = u_t - u_{t-1}$. 
% The special cases are: 
% \begin{itemize}
%     \item When a card with rank 5 is played successfully the number of hint tokens increases by one, if the number of hint tokens is not already at its maximum.
%     \item When the deck is emptied (by a \textit{play} or \textit{discard} action at $d_{t-1} = 1$), the value $c_t$ drops down to zero. Any left over hint tokens cannot be used before the deck is empty, anymore. 
%     The number of undisclosed hints is already at zero when $d_{t-1} = 1$, so it does not change. 
%     \item When the deck is already empty, any action only decreases $p_t$ by one (and increases $t$). It has no influence on $c_t$, $d_t$ or $u_t$, which are all at zero already.
% \end{itemize}



\begin{table}[]
\centering
\begin{threeparttable}[t]
\caption{Effect of actions on the different values.\\The three exceptions at the bottom have priority over the three standard actions at the top.}
\label{tab:action-effects}
\setlength\tabcolsep{4pt}%
\begin{tabular}{l|lllll|l}
action $a_t$ & $\Delta t$ & $\Delta c_t$ & $\Delta d_t$ & $\Delta u_t$ & $\Delta p_t$ & $\Delta\Sigma_t$ \\ \hline \rule{0pt}{2.3ex}%
play    & $+1$ & $0$   & $-1$  & $-1$  & $0$  & $-1$  \\
discard & $+1$ & $+1$  & $-1$  &  $-1$ & $0$  & $0$  \\
hint    & $+1$ & $-1$  &  $0$  &  $0$  & $0$  & $0$ \\ \hline \rule{0pt}{2.3ex}%
% special cases: & & & & & & \\
play a rank 5 successfully *
& $+1$ & $+1$ & $-1$ & $-1$ & $0$ & $0$ \\
$a_t$ empties the deck & $+1$ & $- c_{t-1}$ & $-1$  &  $0$ & $0$  & $\leq 0$  \\
$a_t$ while the deck is empty & $+1$ & $0$ & $0$  & $0$  & $-1$   &  $0$ \\
\end{tabular}
\begin{tablenotes}
* \footnotesize Only if $d_{t-1} > 1$ (otherwise it counts as an action that empties the deck or happens while the deck is empty) and $m_{t-1} < 8$ (otherwise it counts as a normal play action, since we do not gain a hint token with a rank 5 card if the hint budget is already full).
\end{tablenotes}
\end{threeparttable}
\end{table}
% finally found a nice way for a tablefootnote in two-column environment: https://latex.org/forum/viewtopic.php?t=20518



We see that the value of $\Sigma_t$ can never increase during a game. Furthermore, the values $t$, $d_t$, $p_t$, and $m_t$ must always stay non-negative according to the rules of Hanabi. This also implies that the values of $c_t$ and $u_t$ must always be non-negative, since $m_t$ and $d_t$ in \eqref{ctdef} and \eqref{utdef} are non-negative and integer. With this information, and from \eqref{eq:sigmat}, we can conclude that we must always have $t \leq \Sigma_t$.

Thus, the maximum value that $t$ could possibly reach is equal to the value of $\Sigma_0$ (before any action has been taken). We compute these starting values for every possible number of players $p$:
% We always have $c_0 = 8$, and with the number of players $p = 2, 3, 4, 5$ the initial deck size after everybody has been given their opening hands is $d_0 = 40, 35, 34, 30$ respectively.
\vspace{-5pt}
\begin{table}[H]
    \centering
    \caption{Starting values of $\Sigma_t$.}
    \label{tab:sigma0}
\vspace{-12pt}
\begin{center}
    \begin{tabular}{c|cccc}
        $p$ & 2 & 3 & 4 & 5 \\ \hline \rule{0pt}{2.3ex}%
        $\Sigma_0$ & 89 & 80 & 79 & 72
    \end{tabular}
\end{center}
\end{table}
\vspace{-12pt}
As shown in Part 1, there is a particular sequence of actions in a Hanabi game, that gives the following outcome:
% \begin{table}[]
% \centering
% \caption{Possible values for a two-player game.}
% \label{tab:two}
\begin{center}
    \begin{tabular}{l|lllll|l}
         & $t$ & $c_t$ & $d_t$ & $u_t$ & $p_t$ & $\Sigma_t$ \\ \hline \rule{0pt}{2.3ex}%
        start  & $0$ & $8$ & $40$ & $39$ & $2$ &  $89$ \\
        end & $89$ & $0$   & $0$ &  $0$ & $0$ & $89$  
    \end{tabular}
\end{center}
% \end{table}
Therefore, the maximum length of a Hanabi game is 89 turns.

\end{proof}





==> sections/b-proof71.tex <==

\section{Part 2 of the proof of Proposition~\ref{71}}
\label{sec:proof71}

To repeat the proposition:

\begin{proposition*}
The maximum length of a perfect Hanabi game is 71 turns.
\end{proposition*}

\begin{proof}

\textit{Part 1.} See Section \ref{sec:game-length} for the first part of this proof.

\textit{Part 2.} 
We use the same values as defined in part 2 of the proof of Proposition~\ref{89}. We will show that the value of $\Sigma_t$ must decrease to at most 71 for a game to finish in a perfect score.

To reach this score of 25, we need at least 25 play actions of course. In Table \ref{tab:action-effects} it is shown that every play action decreases $\Sigma_t$ by 1, aside from a few exceptions. These exceptions are:
\begin{enumerate}[  (1.)]
    \item Play a rank 5 card successfully when the number of hint tokens is less than 8 and the deck is not empty.
    \item Any action that empties the deck when the number of hint tokens is 0.
    \item Any action when the deck is empty.
\end{enumerate}
These exceptions can all be play actions that do not decrease the value of $\Sigma_t$. Let's try to keep $\Sigma_t$ as high as possible (as it represents the maximum number of turns we can reach) while still scoring 25 points. Thus, we need to make sure as many play actions as possible are classified as one of the three exceptions.

A perfect game can end before the deck is empty, on the deck-emptying move, or when it is already empty. Let us investigate the maximum number of exception play moves in all cases.

If the game ends ...
\begin{itemize}
    \item before the deck is empty: we can use exception (1.) five times,
    \item on the deck-emptying move: we can use (1.) four times and (2.) once, 
    \item when the deck is empty: we can use (1.) four times,
    %\footnote{Not five, then the game would be over already.}
    (2.) once, and (3.) $p$ number of times. Recall that $p$ stands for the number of players. 
\end{itemize}

From all these cases, we see that the maximum possible number of exception play moves is $5 + p$. In a two player game, this would mean that 7 play moves do not decrease $\Sigma_t$, while the other $25-7=18$ do. The maximum number of turns in that case is $89 - 18 = 71$. Recall that 89 is the starting value of $\Sigma_t$ in the two player case, see Table \ref{tab:sigma0}.

\begin{table}[H]
\centering
\caption{Maximum potential number of turns.}
\label{tab:perfect-p}
\vspace{-5pt}
\begin{tabular}{c|c}
\# players & maximum value of $\Sigma_t$ at end of perfect game \\ \hline \rule{0pt}{2.3ex}%
2   & $89 - (25 - (5 + 2)) = 71$                   \\
3   & $80 - (25 - (5 + 3)) = 63$                   \\
4   & $79 - (25 - (5 + 4)) = 63$                   \\
5   & $72 - (25 - (5 + 5)) = 57$                  
\end{tabular}
\end{table}
An overview of the maximum potential number of turns for different values of $p$ is shown in Table~\ref{tab:perfect-p}. We see that in the two player case this value is the highest, meaning that no perfect Hanabi game can possibly be longer than 71 turns. In Part 1 we have shown that a perfect game of this length is indeed possible. Therefore, the maximum length of a perfect Hanabi game is 71 turns. 

\end{proof}


